Scalable multi-class sampling via filtered sliced optimal transport

We propose a multi-class point optimization formulation based on continuous Wasserstein barycenters. Our formulation is designed to handle hundreds to thousands of optimization objectives and comes with a practical optimization scheme. We demonstrate the effectiveness of our framework on various sampling applications like stippling, object placement, and Monte-Carlo integration. We a derive multi-class error bound for perceptual rendering error which can be minimized using our optimization. We provide source code at https://github.com/iribis/filtered-sliced-optimal-transport.

==> figures/progressive_sampling.tex <==
%!TEX root = ../paper.tex

\newcommand{\OneImage}[1]{
    \begin{scope}
        \clip (0,0)-- (0.0,4.5) -- (5.4,4.5) -- (5.4,0.0) -- cycle;
        \path[fill overzoom image=figures/#1] (0,0) rectangle (5.4,4.5);
        
    \end{scope}
}
\newcommand{\ProgressivePlotTwo}[2]{
    \begin{scope}
        \clip (0.0,0.0) -- (5.4,0.0) -- (5.4,4.5) -- (0.0,4.5) -- cycle;
        \path[fill overzoom image=figures//#1] (0,0) rectangle (5.4cm,4.5cm);
    \end{scope}
    \begin{scope}
        \clip (0.9,0.6) -- (2.2,0.6) -- (2.2,2.2) -- (0.9,2.2) -- cycle;
        \path[fill overzoom image=figures//#2] (0.9,0.6) rectangle (2.2cm,2.0cm);
    \end{scope}
    \begin{scope}
        \draw[black,thick] (0.9,0.6) -- (2.2,0.6) -- (2.2,2.0) -- (0.9,2.0) -- cycle;
    \end{scope}
}



\small
\hspace*{-2mm}
\begin{tabular}{c@{}c@{}}

\begin{tikzpicture}[scale=0.8]
    \ProgressivePlotTwo{progressive_sampling/graph_progressive_sampling_WSOT_gaussian_v2.pdf}{progressive_sampling/gaussian.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=0.8]
    \ProgressivePlotTwo{progressive_sampling/graph_progressive_sampling_WSOT_step.pdf}{progressive_sampling/step.png}
\end{tikzpicture}
\end{tabular}


==> figures/reconstruction-problem.tex <==
%!TEX root = ../paper.tex

\definecolor{OutlineColor1}{gray}{0.23}
\definecolor{OutlineColor2}{gray}{0.23}

\newcommand{\OneImage}[1]{
    \begin{scope}
        \clip (0.0,0.0) -- (9.5,0.0) -- (9.5,4.5) -- (0.0,4.5) -- cycle;
        \path[fill overzoom image=figures/#1] (0,0) rectangle (9.5cm,4.5cm);
    \end{scope}
}

\newcommand{\TestVeachImage}[2]{
    %%% Top row
    \begin{scope}
        \clip (0.0,4.5) -- (9.5,4.5) -- (9.5,7) -- (0.0,7) -- cycle;
        \path[fill overzoom image=figures/veach_mis/#1.jpg] (0,0) rectangle (9.5cm,7cm);
    \end{scope}
    \begin{scope}
        \clip (0.0,0.0) -- (9.5,0.0) -- (9.5,4.5) -- (0.0,4.5) -- cycle;
        \path[fill overzoom image=figures/veach_mis/#2.jpg] (0,0) rectangle (9.5cm,7cm);
    \end{scope}

    \begin{scope}
       \draw[draw=white,ultra thick] (0.0,4.5) -- (9.5,4.5);
       \draw[draw=white,ultra thick] (0.0,2.1) -- (9.5,2.1);
       \draw[draw=white,ultra thick] (2.5,0) -- (2.5,4.5);
      \draw[draw=white,ultra thick] (5,0) -- (5,2.1);
    \end{scope}
}

% \newcommand{\VeachImage}[6]{
%     %%% Top row
%     \begin{scope}
%         \clip (0.0,4.5) -- (9.5,4.5) -- (9.5,7) -- (0.0,7) -- cycle;
%         \path[fill overzoom image=figures/veach_mis/#1.jpg] (0,0) rectangle (9.5cm,7cm);
%     \end{scope}
%     %%% Middle row, first col
%     \begin{scope}
%         \clip (0.0,2.1) -- (2.5,2.1) -- (2.5,4.5) -- (0.0,4.5) -- cycle;
%         \path[fill overzoom image=figures/veach_mis/#2.jpg] (0,0) rectangle (9.5cm,7cm);
%     \end{scope}
%     %%% Middle row, second col
%     \begin{scope}
%         \clip (2.5,2.1) -- (9.5,2.1) -- (9.5,4.5) -- (2.5,4.5) -- cycle;
%         \path[fill overzoom image=figures/veach_mis/#3.jpg] (0,0) rectangle (9.5cm,7cm);
%     \end{scope}
%     %%% Bottom row, first col
%     \begin{scope}
%         \clip (0.0,0.0) -- (2.5,0.0) -- (2.5,2.1) -- (0.0,2.1) -- cycle;
%         \path[fill overzoom image=figures/veach_mis/#4.jpg] (0,0) rectangle (9.5cm,7cm);
%     \end{scope}
%     %%% Bottom row, second col
%     \begin{scope}
%         \clip (2.5,0.0) -- (5,0.0) -- (5,2.1) -- (2.5,2.1) -- cycle;
%         \path[fill overzoom image=figures/veach_mis/#5.jpg] (0,0) rectangle (9.5cm,7cm);
%     \end{scope}
%     %%% Bottom row, third col
%     \begin{scope}
%         \clip (5.0,0.0) -- (9.5,0.0) -- (9.5,2.1) -- (5.0,2.1) -- cycle;
%         \path[fill overzoom image=figures/veach_mis/#6.jpg] (0,0) rectangle (9.5cm,7cm);
%     \end{scope}

%     \begin{scope}
%       \draw[draw=white,ultra thick] (0.0,4.5) -- (9.5,4.5);
%       \draw[draw=white,ultra thick] (0.0,2.1) -- (9.5,2.1);
%       \draw[draw=white,ultra thick] (2.5,0) -- (2.5,4.5);
%       \draw[draw=white,ultra thick] (5,0) -- (5,2.1);
%     \end{scope}
% }



\newcommand{\VeachCrop}[5]{
    \begin{scope}
        \clip (#1,#2) -- (#3,#2) -- (#3,#4) -- (#1,#4) -- cycle;
        \path[fill overzoom image=figures/veach_mis/#5.jpg] (0,0) rectangle (9.5cm,7cm);
    \end{scope}
}

\newcommand{\VeachImage}[6]{
    % %%% Top row
    % \begin{scope}
    %     \clip (0.0,4.5) -- (9.5,4.5) -- (9.5,7) -- (0.0,7) -- cycle;
    %     \path[fill overzoom image=figures/veach_mis/#1.jpg] (0,0) rectangle (9.5cm,7cm);
    % \end{scope}
    %%% Middle row, first col
    \begin{scope}
        \clip (0.0,0.0) -- (2.5,0.0) -- (2.5,7) -- (0.0,7) -- cycle;
        \path[fill overzoom image=figures/veach_mis/#2.jpg] (0,0) rectangle (9.5cm,7cm);
    \end{scope}
    %%% Middle row, second col
    \begin{scope}
        \clip (2.5,2.1) -- (9.5,2.1) -- (9.5,7) -- (2.5,7) -- cycle;
        \path[fill overzoom image=figures/veach_mis/#3.jpg] (0,0) rectangle (9.5cm,7cm);
    \end{scope}
    %%% Bottom row, first col
    % \begin{scope}
    %     \clip (0.0,0.0) -- (2.5,0.0) -- (2.5,2.1) -- (0.0,2.1) -- cycle;
    %     \path[fill overzoom image=figures/veach_mis/#4.jpg] (0,0) rectangle (9.5cm,7cm);
    % \end{scope}
    %%% Bottom row, second col
    \begin{scope}
        \clip (2.5,0.0) -- (5,0.0) -- (5,2.1) -- (2.5,2.1) -- cycle;
        \path[fill overzoom image=figures/veach_mis/#5.jpg] (0,0) rectangle (9.5cm,7cm);
    \end{scope}
    %%% Bottom row, third col
    \begin{scope}
        \clip (5.0,0.0) -- (9.5,0.0) -- (9.5,2.1) -- (5.0,2.1) -- cycle;
        \path[fill overzoom image=figures/veach_mis/#6.jpg] (0,0) rectangle (9.5cm,7cm);
    \end{scope}

    \begin{scope}
    %   \draw[draw=white,ultra thick] (0.0,4.5) -- (9.5,4.5);
    %   \draw[draw=white,ultra thick] (0.0,2.1) -- (9.5,2.1);
    %   \draw[draw=white,ultra thick] (2.5,0) -- (2.5,4.5);
    %   \draw[draw=white,ultra thick] (5,0) -- (5,2.1);
    \end{scope}
}

\small
\hspace*{-2.3mm}
\begin{tabular}{c@{}}
\begin{tikzpicture}[scale=0.9]
    \OneImage{reconstruction-problem.ai}
    \begin{scope}
        \filldraw[black,ultra thick] (1.25, -0.2) circle (0pt) node[anchor=base,rotate=0]{\fontsize{7.3}{6}\selectfont (a)\,Box reconst.};
        %
        \filldraw[black,ultra thick] (3.77, -0.2) circle (0pt) node[anchor=base,rotate=0]{\fontsize{7.3}{6}\selectfont (b)\,Gaussian reconst.};
        %
        \filldraw[black,ultra thick] (7.26, -0.2) circle (0pt) node[anchor=base,rotate=0]{\fontsize{7.3}{6}\selectfont (c)\,Gaussian reconst.\ + percept.\ filter};
    \end{scope}
    
    \begin{scope}
        \filldraw[black,ultra thick] (1.0, 0.6) circle (0pt) node[anchor=south west,rotate=0]{$\PointSetExt$};
    %   \filldraw[gray,ultra thick] (1.9, 0.2) circle (0pt) node[anchor=south west,rotate=0] {$\Hypercube$};
    %   \filldraw[gray,ultra thick] (4.4, 0.2) circle (0pt) node[anchor=south west,rotate=0] {$\Hypercube$};
    %   \filldraw[gray,ultra thick] (9, 0.2) circle (0pt) node[anchor=south west,rotate=0] {$\Hypercube$};
    \end{scope}
    
    \begin{scope}[overlay]
        \filldraw[black,ultra thick] (-0.2, 2.7) circle (0pt) node[anchor=south west,rotate=0]{\footnotesize\color{ExtSpaceColor}$\Hypercube^2$};
        \filldraw[black,ultra thick] (-0.05, 0.1) circle (0pt) node[anchor=south west,rotate=0]{\footnotesize\color{DomainColor}$\Hypercube^d$};
        \filldraw[black,ultra thick] (0.7, 3.45) circle (0pt) node[anchor=south west,rotate=0]{\footnotesize $\EstimatedImage_\ReconstFilter(\PointSetExt)$};
        \filldraw[black,ultra thick] (3.2, 3.45) circle (0pt) node[anchor=south west,rotate=0]{\footnotesize $\EstimatedImage_\ReconstFilter(\PointSetExt)$};
        \filldraw[black,ultra thick] (6.5, 4.1) circle (0pt) node[anchor=south west,rotate=0]{\footnotesize $\EstimatedImage_{\PerceptFilter * \ReconstFilter}(\PointSetExt)$};
    \end{scope}
    
    \begin{scope}
        \filldraw[black,ultra thick] (0.6, 2.78) circle (0pt) node[anchor=south west,rotate=0]{$\ReconstFilter$};
        \filldraw[black,ultra thick] (3.12, 2.78) circle (0pt) node[anchor=south west,rotate=0]{$\ReconstFilter$};
        \filldraw[black,ultra thick] (7.08, 2.78) circle (0pt) node[anchor=south west,rotate=0]{$\ReconstFilter$};
        \filldraw[black,ultra thick] (7.05, 3.4) circle (0pt) node[anchor=south west,rotate=0]{$\PerceptFilter$};
    \end{scope}
        
    \begin{scope}
        \filldraw[black,ultra thick] (3, 4.25) circle (0pt) node[anchor=south west,rotate=0]{\scriptsize Perceived image};
        \filldraw[black,ultra thick] (2.5, 4.0) circle (0pt) node[anchor=south west,rotate=0]{\scriptsize Reconstructed image};
        
        \draw[gray, ->] (4.5,4.0) -- (5.05,3.4);
        \draw[gray, ->] (4.8,4.4) -- (5.05,4.1);
    \end{scope}
    
    % \begin{overpic}[abs,unit=0.25mm]{figures/reconstruction-problem-inverted.pdf}
\end{tikzpicture}
\\
% \rotatebox{90}{\quad Global ours \qquad Per-pixel ours \qquad\quad QMC}
\newcommand{\SplitOne}{2.7}%
\newcommand{\SplitTwo}{4.75}%
\newcommand{\SplitThree}{6.8}%
\begin{tikzpicture}[scale=0.9]
    % \VeachImage
    %     {veach-mis_low_res_directlight_halton_n4_gaussian_no-perceptual}
    %     {veach-mis_low_res_directlight_Ours_n4_box_no-perceptual}
    %     {veach-mis_low_res_directlight_Ours_n4_gaussian_no-perceptual_independant_pixels}
    %     {veach-mis_low_res_directlight_Ours_n4_box_no-perceptual}
    %     {veach-mis_low_res_directlight_Ours_n4_gaussian_no-perceptual}
    %     {veach-mis_low_res_directlight_Ours_n4_gaussian_perceptual}
    \VeachCrop{0}{0}{\SplitOne}{7.8}{veach-mis_low_res_directlight_Ours_n4_box_no-perceptual}
    \VeachCrop{\SplitOne}{0}{\SplitTwo}{7.8}{veach-mis_low_res_directlight_Ours_n4_gaussian_no-perceptual_independant_pixels}
    \VeachCrop{\SplitTwo}{0}{\SplitThree}{7.8}{veach-mis_low_res_directlight_Ours_n4_gaussian_no-perceptual}
    \VeachCrop{\SplitThree}{0}{9.5}{7.8}{veach-mis_low_res_directlight_Ours_n4_gaussian_perceptual}
    \begin{scope}[overlay]
        \fill [black,opacity=0.4] (0,7.4) rectangle (9.5,7.8);
        \fill [black,opacity=0.3] (0,7) rectangle (9.5,7.4);
        %
        \draw[draw=black,line width=0.15mm] (\SplitOne,0) -- (\SplitOne,7.8);
        \draw[draw=black,line width=0.15mm] (\SplitTwo,0) -- (\SplitTwo,7.4);
        \draw[draw=black,line width=0.15mm] (\SplitThree,0) -- (\SplitThree,7.4);
        %
        \filldraw[black,ultra thick] (1.35, 7.5) circle (0pt)  node[anchor=base,rotate=0]{\fontsize{8}{6}\selectfont \Outlined[white][OutlineColor1][0.7pt]{Box reconstuction}};
        \filldraw[black,ultra thick] (1.35, 7.12) circle (0pt)  node[anchor=base,rotate=0]{\fontsize{7}{6}\selectfont \Outlined[white][OutlineColor2][0.65pt]{(d)\,Box optimization}};
        %
        % \filldraw[black,ultra thick] (3.725, 7.5) circle (0pt)  node[anchor=base,rotate=0]{\fontsize{7}{6}\selectfont \Outlined[white][OutlineColor1][0.7pt]{Gaussian reconst.}};
        \filldraw[black,ultra thick] (3.725, 7.12) circle (0pt)  node[anchor=base,rotate=0]{\fontsize{7}{6}\selectfont \Outlined[white][OutlineColor2][0.65pt]{(e)\,Box\,optim.}};
        %
        \filldraw[black,ultra thick] (5.775, 7.5) circle (0pt)  node[anchor=base,rotate=0]{\fontsize{8}{6}\selectfont \Outlined[white][OutlineColor1][0.7pt]{Gaussian reconstruction}};
        \filldraw[black,ultra thick] (5.775, 7.12) circle (0pt)  node[anchor=base,rotate=0]{\fontsize{7}{6}\selectfont \Outlined[white][OutlineColor2][0.65pt]{(f)\,Gaussian\,opt.}};
        %
        % \filldraw[black,ultra thick] (8.15, 7.5) circle (0pt)  node[anchor=base,rotate=0]{\fontsize{7}{6}\selectfont \Outlined[white][black][0.7pt]{Gaussian reconst.}};
        \filldraw[black,ultra thick] (8.15, 7.12) circle (0pt)  node[anchor=base,rotate=0]{\fontsize{7}{6}\selectfont \Outlined[white][OutlineColor2][0.65pt]{(g)\,Gauss.+percep.\,opt.}};
    \end{scope}
\end{tikzpicture}%
\end{tabular}






% %!TEX root = ../paper.tex

% \definecolor{OutlineColor2}{gray}{0.25}

% \newcommand{\OneImage}[1]{
%     \begin{scope}
%         \clip (0.0,0.0) -- (9.5,0.0) -- (9.5,4.5) -- (0.0,4.5) -- cycle;
%         \path[fill overzoom image=figures/#1] (0,0) rectangle (9.5cm,4.5cm);
%     \end{scope}
% }

% \newcommand{\TestVeachImage}[2]{
%     %%% Top row
%     \begin{scope}
%         \clip (0.0,4.5) -- (9.5,4.5) -- (9.5,7) -- (0.0,7) -- cycle;
%         \path[fill overzoom image=figures/veach_mis/#1.jpg] (0,0) rectangle (9.5cm,7cm);
%     \end{scope}
%     \begin{scope}
%         \clip (0.0,0.0) -- (9.5,0.0) -- (9.5,4.5) -- (0.0,4.5) -- cycle;
%         \path[fill overzoom image=figures/veach_mis/#2.jpg] (0,0) rectangle (9.5cm,7cm);
%     \end{scope}

%     \begin{scope}
%       \draw[draw=white,ultra thick] (0.0,4.5) -- (9.5,4.5);
%       \draw[draw=white,ultra thick] (0.0,2.1) -- (9.5,2.1);
%       \draw[draw=white,ultra thick] (2.5,0) -- (2.5,4.5);
%       \draw[draw=white,ultra thick] (5,0) -- (5,2.1);
%     \end{scope}
% }

% % \newcommand{\VeachImage}[6]{
% %     %%% Top row
% %     \begin{scope}
% %         \clip (0.0,4.5) -- (9.5,4.5) -- (9.5,7) -- (0.0,7) -- cycle;
% %         \path[fill overzoom image=figures/veach_mis/#1.jpg] (0,0) rectangle (9.5cm,7cm);
% %     \end{scope}
% %     %%% Middle row, first col
% %     \begin{scope}
% %         \clip (0.0,2.1) -- (2.5,2.1) -- (2.5,4.5) -- (0.0,4.5) -- cycle;
% %         \path[fill overzoom image=figures/veach_mis/#2.jpg] (0,0) rectangle (9.5cm,7cm);
% %     \end{scope}
% %     %%% Middle row, second col
% %     \begin{scope}
% %         \clip (2.5,2.1) -- (9.5,2.1) -- (9.5,4.5) -- (2.5,4.5) -- cycle;
% %         \path[fill overzoom image=figures/veach_mis/#3.jpg] (0,0) rectangle (9.5cm,7cm);
% %     \end{scope}
% %     %%% Bottom row, first col
% %     \begin{scope}
% %         \clip (0.0,0.0) -- (2.5,0.0) -- (2.5,2.1) -- (0.0,2.1) -- cycle;
% %         \path[fill overzoom image=figures/veach_mis/#4.jpg] (0,0) rectangle (9.5cm,7cm);
% %     \end{scope}
% %     %%% Bottom row, second col
% %     \begin{scope}
% %         \clip (2.5,0.0) -- (5,0.0) -- (5,2.1) -- (2.5,2.1) -- cycle;
% %         \path[fill overzoom image=figures/veach_mis/#5.jpg] (0,0) rectangle (9.5cm,7cm);
% %     \end{scope}
% %     %%% Bottom row, third col
% %     \begin{scope}
% %         \clip (5.0,0.0) -- (9.5,0.0) -- (9.5,2.1) -- (5.0,2.1) -- cycle;
% %         \path[fill overzoom image=figures/veach_mis/#6.jpg] (0,0) rectangle (9.5cm,7cm);
% %     \end{scope}

% %     \begin{scope}
% %       \draw[draw=white,ultra thick] (0.0,4.5) -- (9.5,4.5);
% %       \draw[draw=white,ultra thick] (0.0,2.1) -- (9.5,2.1);
% %       \draw[draw=white,ultra thick] (2.5,0) -- (2.5,4.5);
% %       \draw[draw=white,ultra thick] (5,0) -- (5,2.1);
% %     \end{scope}
% % }



% \newcommand{\VeachCrop}[5]{
%     \begin{scope}
%         \clip (#1,#2) -- (#3,#2) -- (#3,#4) -- (#1,#4) -- cycle;
%         \path[fill overzoom image=figures/veach_mis/#5.jpg] (0,0) rectangle (9.5cm,7cm);
%     \end{scope}
% }

% \newcommand{\VeachImage}[6]{
%     % %%% Top row
%     % \begin{scope}
%     %     \clip (0.0,4.5) -- (9.5,4.5) -- (9.5,7) -- (0.0,7) -- cycle;
%     %     \path[fill overzoom image=figures/veach_mis/#1.jpg] (0,0) rectangle (9.5cm,7cm);
%     % \end{scope}
%     %%% Middle row, first col
%     \begin{scope}
%         \clip (0.0,0.0) -- (2.5,0.0) -- (2.5,7) -- (0.0,7) -- cycle;
%         \path[fill overzoom image=figures/veach_mis/#2.jpg] (0,0) rectangle (9.5cm,7cm);
%     \end{scope}
%     %%% Middle row, second col
%     \begin{scope}
%         \clip (2.5,2.1) -- (9.5,2.1) -- (9.5,7) -- (2.5,7) -- cycle;
%         \path[fill overzoom image=figures/veach_mis/#3.jpg] (0,0) rectangle (9.5cm,7cm);
%     \end{scope}
%     %%% Bottom row, first col
%     % \begin{scope}
%     %     \clip (0.0,0.0) -- (2.5,0.0) -- (2.5,2.1) -- (0.0,2.1) -- cycle;
%     %     \path[fill overzoom image=figures/veach_mis/#4.jpg] (0,0) rectangle (9.5cm,7cm);
%     % \end{scope}
%     %%% Bottom row, second col
%     \begin{scope}
%         \clip (2.5,0.0) -- (5,0.0) -- (5,2.1) -- (2.5,2.1) -- cycle;
%         \path[fill overzoom image=figures/veach_mis/#5.jpg] (0,0) rectangle (9.5cm,7cm);
%     \end{scope}
%     %%% Bottom row, third col
%     \begin{scope}
%         \clip (5.0,0.0) -- (9.5,0.0) -- (9.5,2.1) -- (5.0,2.1) -- cycle;
%         \path[fill overzoom image=figures/veach_mis/#6.jpg] (0,0) rectangle (9.5cm,7cm);
%     \end{scope}

%     \begin{scope}
%     %   \draw[draw=white,ultra thick] (0.0,4.5) -- (9.5,4.5);
%     %   \draw[draw=white,ultra thick] (0.0,2.1) -- (9.5,2.1);
%     %   \draw[draw=white,ultra thick] (2.5,0) -- (2.5,4.5);
%     %   \draw[draw=white,ultra thick] (5,0) -- (5,2.1);
%     \end{scope}
% }

% \small
% \hspace*{-2.3mm}
% \begin{tabular}{c@{}}
% \begin{tikzpicture}[scale=0.9]
%     \OneImage{reconstruction-problem.ai}
%     \begin{scope}
%         \filldraw[black,ultra thick] (1.25, -0.2) circle (0pt) node[anchor=base,rotate=0]{\fontsize{7.3}{6}\selectfont (a)\,Box reconst.};
%         %
%         \filldraw[black,ultra thick] (3.77, -0.2) circle (0pt) node[anchor=base,rotate=0]{\fontsize{7.3}{6}\selectfont (b)\,Gaussian reconst.};
%         %
%         \filldraw[black,ultra thick] (7.26, -0.2) circle (0pt) node[anchor=base,rotate=0]{\fontsize{7.3}{6}\selectfont (c)\,Gaussian reconst.\ + percept.\ filter};
%     \end{scope}
    
%     \begin{scope}
%         \filldraw[black,ultra thick] (1.0, 0.6) circle (0pt) node[anchor=south west,rotate=0]{$\PointSetExt$};
%     %   \filldraw[gray,ultra thick] (1.9, 0.2) circle (0pt) node[anchor=south west,rotate=0] {$\Hypercube$};
%     %   \filldraw[gray,ultra thick] (4.4, 0.2) circle (0pt) node[anchor=south west,rotate=0] {$\Hypercube$};
%     %   \filldraw[gray,ultra thick] (9, 0.2) circle (0pt) node[anchor=south west,rotate=0] {$\Hypercube$};
%     \end{scope}
    
%     \begin{scope}[overlay]
%         \filldraw[black,ultra thick] (-0.2, 2.7) circle (0pt) node[anchor=south west,rotate=0]{\footnotesize\color{ExtSpaceColor}$\Hypercube^2$};
%         \filldraw[black,ultra thick] (-0.05, 0.1) circle (0pt) node[anchor=south west,rotate=0]{\footnotesize\color{DomainColor}$\Hypercube^d$};
%         \filldraw[black,ultra thick] (0.7, 3.45) circle (0pt) node[anchor=south west,rotate=0]{\footnotesize $\EstimatedImage_\ReconstFilter(\PointSetExt)$};
%         \filldraw[black,ultra thick] (3.2, 3.45) circle (0pt) node[anchor=south west,rotate=0]{\footnotesize $\EstimatedImage_\ReconstFilter(\PointSetExt)$};
%         \filldraw[black,ultra thick] (6.5, 4.1) circle (0pt) node[anchor=south west,rotate=0]{\footnotesize $\EstimatedImage_{\PerceptFilter * \ReconstFilter}(\PointSetExt)$};
%     \end{scope}
    
%     \begin{scope}
%         \filldraw[black,ultra thick] (0.6, 2.78) circle (0pt) node[anchor=south west,rotate=0]{$\ReconstFilter$};
%         \filldraw[black,ultra thick] (3.12, 2.78) circle (0pt) node[anchor=south west,rotate=0]{$\ReconstFilter$};
%         \filldraw[black,ultra thick] (7.08, 2.78) circle (0pt) node[anchor=south west,rotate=0]{$\ReconstFilter$};
%         \filldraw[black,ultra thick] (7.05, 3.4) circle (0pt) node[anchor=south west,rotate=0]{$\PerceptFilter$};
%     \end{scope}
        
%     \begin{scope}
%         \filldraw[black,ultra thick] (3, 4.25) circle (0pt) node[anchor=south west,rotate=0]{\scriptsize Perceived image};
%         \filldraw[black,ultra thick] (2.5, 4.0) circle (0pt) node[anchor=south west,rotate=0]{\scriptsize Reconstructed image};
        
%         \draw[gray, ->] (4.5,4.0) -- (5.05,3.4);
%         \draw[gray, ->] (4.8,4.4) -- (5.05,4.1);
%     \end{scope}
    
%     % \begin{overpic}[abs,unit=0.25mm]{figures/reconstruction-problem-inverted.pdf}
% \end{tikzpicture}
% \\
% % \rotatebox{90}{\quad Global ours \qquad Per-pixel ours \qquad\quad QMC}
% \newcommand{\SplitOne}{2.7}%
% \newcommand{\SplitTwo}{4.75}%
% \newcommand{\SplitThree}{6.8}%
% \begin{tikzpicture}[scale=0.9]
%     % \VeachImage
%     %     {veach-mis_low_res_directlight_halton_n4_gaussian_no-perceptual}
%     %     {veach-mis_low_res_directlight_Ours_n4_box_no-perceptual}
%     %     {veach-mis_low_res_directlight_Ours_n4_gaussian_no-perceptual_independant_pixels}
%     %     {veach-mis_low_res_directlight_Ours_n4_box_no-perceptual}
%     %     {veach-mis_low_res_directlight_Ours_n4_gaussian_no-perceptual}
%     %     {veach-mis_low_res_directlight_Ours_n4_gaussian_perceptual}
%     \VeachCrop{0}{0}{\SplitOne}{7}{veach-mis_low_res_directlight_Ours_n4_box_no-perceptual}
%     \VeachCrop{\SplitOne}{0}{\SplitTwo}{7}{veach-mis_low_res_directlight_Ours_n4_gaussian_no-perceptual_independant_pixels}
%     \VeachCrop{\SplitTwo}{0}{\SplitThree}{7}{veach-mis_low_res_directlight_Ours_n4_gaussian_no-perceptual}
%     \VeachCrop{\SplitThree}{0}{9.5}{7}{veach-mis_low_res_directlight_Ours_n4_gaussian_perceptual}
%     \begin{scope}[overlay]
%         \fill [black,opacity=0.6] (0,6.6) rectangle (9.5,7);
%         \fill [black,opacity=0.3] (0,6.2) rectangle (9.5,6.6);
%         %
%         \draw[draw=black,line width=0.15mm] (\SplitOne,0) -- (\SplitOne,7);
%         \draw[draw=black,line width=0.15mm] (\SplitTwo,0) -- (\SplitTwo,6.6);
%         \draw[draw=black,line width=0.15mm] (\SplitThree,0) -- (\SplitThree,6.6);
%         %
%         \filldraw[black,ultra thick] (1.35, 6.7) circle (0pt)  node[anchor=base,rotate=0]{\fontsize{8}{6}\selectfont \Outlined[white][black][0.7pt]{Box reconstuction}};
%         \filldraw[black,ultra thick] (1.35, 6.32) circle (0pt)  node[anchor=base,rotate=0]{\fontsize{7}{6}\selectfont \Outlined[white][OutlineColor2][0.65pt]{(d)\,Box optimization}};
%         %
%         % \filldraw[black,ultra thick] (3.725, 6.7) circle (0pt)  node[anchor=base,rotate=0]{\fontsize{7}{6}\selectfont \Outlined[white][black][0.7pt]{Gaussian reconst.}};
%         \filldraw[black,ultra thick] (3.725, 6.32) circle (0pt)  node[anchor=base,rotate=0]{\fontsize{7}{6}\selectfont \Outlined[white][OutlineColor2][0.65pt]{(e)\,Box\,optim.}};
%         %
%         \filldraw[black,ultra thick] (5.775, 6.7) circle (0pt)  node[anchor=base,rotate=0]{\fontsize{8}{6}\selectfont \Outlined[white][black][0.7pt]{Gaussian reconstruction}};
%         \filldraw[black,ultra thick] (5.775, 6.32) circle (0pt)  node[anchor=base,rotate=0]{\fontsize{7}{6}\selectfont \Outlined[white][OutlineColor2][0.65pt]{(f)\,Gaussian\,opt.}};
%         %
%         % \filldraw[black,ultra thick] (8.15, 6.7) circle (0pt)  node[anchor=base,rotate=0]{\fontsize{7}{6}\selectfont \Outlined[white][black][0.7pt]{Gaussian reconst.}};
%         \filldraw[black,ultra thick] (8.15, 6.32) circle (0pt)  node[anchor=base,rotate=0]{\fontsize{7}{6}\selectfont \Outlined[white][OutlineColor2][0.65pt]{(g)\,Gauss.+percep.\,opt.}};
%     \end{scope}
% \end{tikzpicture}%
% \end{tabular}


==> figures/teaser.tex <==
%!TEX root = ../paper.tex

\newcommand{\OneImage}[1]{
    \begin{scope}
        \clip (0,0) -- (8.5,0) -- (8.5,4.5) -- (0,4.5) -- cycle;
        \path[fill overzoom image=figures/#1] (0,0) rectangle (8.5cm,4.5cm);
        
    \end{scope}
}

\newcommand{\VerticalSplitTwoImages}[2]{
    \begin{scope}
        \clip (0,0)-- (0.0,4.5) -- (4.25,4.5) -- (4.25,0.0) -- cycle;
        \path[fill overzoom image=figures/#1] (0,0) rectangle (8.5,4.5);
    \end{scope}
    \begin{scope}
        \clip (4.25,0.0)-- (4.25,4.5) -- (8.5,4.5) -- (8.5,0.0) -- cycle;
        \path[fill overzoom image=figures/#2] (0,0) rectangle (8.5,4.5);
    \end{scope}
    \draw[draw=white,thick] (3.25,4.5) -- (5.25,0.0);
    %\draw[draw=white,thin] (0,0.5) -- (1,0.5);
}

\newcommand{\SlantedSplitTwoImages}[2]{
    \begin{scope}
        \clip (0,0)-- (0.0,4.5) -- (5.25,4.5) -- (3.25,0.0) -- cycle;
        \path[fill overzoom image=figures/#1] (0,0) rectangle (8.5,4.5);
    \end{scope}
    \begin{scope}
        \clip (3.25,0.0)-- (5.25,4.5) -- (8.5,4.5) -- (8.5,0.0) -- cycle;
        \path[fill overzoom image=figures/#2] (0,0) rectangle (8.5,4.5);
    \end{scope}
    \draw[draw=white,thick] (5.25,4.5) -- (3.25,0.0);
    %\draw[draw=white,thin] (0,0.5) -- (1,0.5);
}

\newcommand{\TwoImagesSmall}[2]{
    \begin{scope}
        \clip (0,0)-- (0.0,4.5) -- (3.25,4.5) -- (3.25,0.0) -- cycle;
        \path[fill overzoom image=figures/#1] (0,0) rectangle (6.5,4.5);
    \end{scope}
    \begin{scope}
        \clip (3.25,0.0)-- (3.25,4.5) -- (8.5,4.5) -- (6.5,0.0) -- cycle;
        \path[fill overzoom image=figures/#2] (0,0) rectangle (6.5,4.5);
    \end{scope}
    \draw[draw=white,thick] (3.25,4.5) -- (3.25,0.0);
    %\draw[draw=white,thin] (0,0.5) -- (1,0.5);
}


\small
\hspace*{-2mm}
\begin{tabular}{c@{\;}c@{}}
    \begin{tikzpicture}[scale=1.05]
        \OneImage{stipling/beach/beach_cmyk.png}
    \end{tikzpicture}
    %     &
    % \begin{tikzpicture}[scale=0.8]
    %     \OneImage{teaser/test_object_placement.png}
    % \end{tikzpicture}
        &
    \begin{tikzpicture}[scale=1.05]
        \SlantedSplitTwoImages{teaser/chopper-titan_directlight_random_n1_gaussian_perceptual.jpg}{teaser/chopper-titan_directlight_Ours_n1_gaussian_perceptual.jpg}
        \begin{scope}
            \filldraw[white,ultra thick] (0.3, 4.4) circle (0pt) node[anchor=north,rotate=0] 
            {MC \tiny};
            \filldraw[white,ultra thick] (8.0, 4.4) circle (0pt) node[anchor=north,rotate=0] 
            {Ours \tiny};
        \end{scope}
    \end{tikzpicture}
    \\
    Color stippling & Blue-noise error distribution
\end{tabular}
